Multi-Objective Amortized CDRH3 Sequence Sampling Diversifies Promising Antibody Candidates

Antibody therapeutics have transformed treatment across diverse therapeutic areas and have become central to modern medicine. While recent machine learning approaches aim to accelerate antibody discovery through structure-based design and target-affinity optimization, successful candidates must also satisfy broad developability constraints, including structural compatibility, low immunogenicity, and favorable biophysical properties, while remaining sufficiently diverse to provide sufficient coverage of design space to mitigate later-stage development failures. We introduce a preference-conditioned multi-objective generative flow network (GFN) fine-tuning pipeline for fixed-framework CDRH3 loop redesign that fine-tunes a biological sequence model against many inexpensive proxies covering backbone compatibility, sequence likelihood, immunogenicity risk, novelty, and developability liabilities. It combines up to fourteen predictive rewards in a single policy trained to sample CDRH3 loops across 623 SAbDab antibody structures, leveraging a reward reduction strategy to preserve Pareto dominance under this learned map. We also introduce a novel autoregressive span-in-filling variant of AMPLIFY-350M that serves both as a scaffold-conditioned CDRH3 generation prior and as a direct conditional likelihood scorer. We evaluated reward scores, diversity, and design quality on loops sampled on 45 held-out antibody complexes to assess structural consistency, confidence, aggregation propensity, stability, and antigen binding. Compared with the inverse-folding methods ProteinMPNN and ESM-IF, our approach produces roughly 10x more distinct acceptable candidates per design at 50% sequence identity, while holding 10% of the 14-objective Pareto front pooled across methods, trading per-sample quality for greater exploration of novel possible structures.

==> tables/backbone_validation_dms.tex <==
% GENERATED by paper/scripts/make_backbone_validation_tables.py -- DO NOT EDIT.
\begin{table}[!htb]
\centering
\caption{Zero-shot fitness prediction on ProteinGym v1.3 substitutions, restricted to the 162 assays whose protein is at most 512 residues. Spearman $\rho$ between predicted and measured mutational effect, averaged over assays within each length band. \textbf{The restriction is to the regime this backbone is used in}: the antibody task runs at 110--242 residues (244 tokens once rearranged for in-filling), so every one of the 784 structures sits inside even the 512-token context that 95\% of pretraining used. Longer assays would measure a regime the pipeline never enters, and would confound the objective comparison with a context-extension effect. Note the restriction is the \emph{less} flattering choice --- the in-filling model's deficit is larger on short proteins than on long ones. \textbf{Both models are scored here, on the same download}, rather than against a published figure, so nothing depends on matching a benchmark version or an aggregation convention. The estimators are matched in cost and information: one forward per mutated \emph{position} gives the full residue distribution there, from an end-anchored in-filling span or a masked marginal, and mutant scores are the standard additive $\sum_i [\log p(\mathrm{mut}_i) - \log p(\mathrm{wt}_i)]$.}
\label{tab:backbone-validation-dms}
\small
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Protein length & assays & in-filling & masked & $\Delta$ & in-filling wins \\
\midrule
$\leq$256 & 112 & +0.273 & +0.410 & -0.137 & 13 \\
257--512 & 50 & +0.333 & +0.396 & -0.063 & 7 \\
\midrule
\textbf{all} & \textbf{162} & \textbf{+0.292} & \textbf{+0.406} & \textbf{-0.114} & \textbf{20} \\
\bottomrule
\end{tabular}
\\[3pt] \footnotesize Paired Wilcoxon signed-rank test over assays: $p = 3.5e-22$.
\end{table}


==> tables/backbone_validation_loss.tex <==
% GENERATED by paper/scripts/make_backbone_validation_tables.py -- DO NOT EDIT.
\begin{table}[!htb]
\centering
\caption{Held-out span-in-filling loss. Spans are drawn the way the training collator drew them (length uniform on $[1,50]$ clamped by the sequence{,} uniform start){,} at context length 2048. \textbf{The reproduction column is the check that this evaluation measures what training measured}: it is the pretraining log's final value for the same set{,} computed by separate code. \texttt{oas\_dev} is the one set where the two disagree{,} because OAS loss is bimodal --- 41\% of spans land in germline-conserved framework and score $\approx$0 while CDR spans score high --- so its mean is a fragile summary of a mixture rather than a stable quantity. The last two rows are the memorization control.}
\label{tab:backbone-validation-loss}
\small
\begin{tabular}{@{}lrrrr@{}}
\toprule
Set & $n$ & NLL/token & perplexity & pretraining log \\
\midrule
\texttt{uniprot\_dev} & 10{,}000 & 1.4074 & 4.085 & 1.4296 \\
\texttt{oas\_dev} & 20{,}000 & 0.4902 & 1.633 & 0.2381 \\
\texttt{scop\_dev} & 10{,}000 & 1.8637 & 6.448 & 1.8970 \\
native CDRH3 (held-out) & 55 & 2.3538 & 10.526 & --- \\
\midrule
\texttt{scop\_train} & 2{,}000 & 1.1271 & 3.087 & --- \\
\texttt{oas\_train} & 2{,}000 & 0.5022 & 1.652 & --- \\
\bottomrule
\end{tabular}
\end{table}


==> tables/backbone_validation_recovery_diff.tex <==
% GENERATED by paper/scripts/make_backbone_validation_tables.py -- DO NOT EDIT.
\begin{table}[!htb]
\centering
\caption{Span recovery against the original masked-language-model AMPLIFY-350M, at matched span length. Recovery is argmax accuracy over the 20 canonical \textcolor{red}{residues.} \textcolor{red}{Note that the exact likelihood calculated under AMPLIFY-AR is not directly comparable to the pseudo-likelihood calculated under the original AMPLIFY.} $\mathrm{AR}_{\mathrm{gen}}$ \textcolor{red}{and} $\mathrm{MLM}_{\mathrm{gen}}$ both generate the span conditioned only on their own \textcolor{red}{predictions.} $\mathrm{AR}_{\mathrm{nat}}$ \textcolor{red}{and} $\mathrm{MLM}_{\mathrm{nat}}$ see native \textcolor{red}{context.} $n$ falls with span length because the $L$-forward decodings cost $O(L)$ for \textcolor{red}{MLM models.} \textcolor{red}{We use the same sequences for all model evaluations.}}
\label{tab:backbone-validation-recovery}
\small
\begin{tabular}{@{}llrrrrrrr@{}}
\toprule
& & & \multicolumn{3}{c}{generation (self-conditioned)} & \multicolumn{2}{c}{native-conditioned} & \\
\cmidrule(lr){4-6}\cmidrule(lr){7-8}
Corpus & $L$ & $n$ & $\mathrm{AR}_{\mathrm{gen}}$ & $\mathrm{MLM}_{\mathrm{gen}}$ & $\Delta$ & $\mathrm{AR}_{\mathrm{nat}}$ & $\mathrm{MLM}_{\mathrm{nat}}$  \\
\midrule
UniProt, $\leq$256 aa & 1 & 2000 & 0.514 & 0.526 & -0.012 & 0.514 & 0.526 \\
 & 2 & 2000 & 0.501 & 0.513 & -0.012 & 0.510 & 0.526 \\
 & 3 & 2000 & 0.485 & 0.507 & -0.021 & 0.502 & 0.525 \\
 & 5 & 2000 & 0.481 & 0.488 & -0.007 & 0.519 & 0.519 \\
 & 8 & 2000 & 0.477 & 0.470 & \textbf{+0.007} & 0.528 & 0.533  \\
 & 13 & 1230 & 0.454 & 0.424 & \textbf{+0.030} & 0.532 & 0.528  \\
 & 21 & 761 & 0.450 & 0.386 & \textbf{+0.064} & 0.553 & 0.543  \\
 & 34 & 470 & 0.400 & 0.304 & \textbf{+0.096} & 0.552 & 0.535  \\
 & 50 & 400 & 0.373 & 0.226 & \textbf{+0.148} & 0.547 & 0.544  \\
\midrule
UniProt, 257--512 aa & 1 & 2000 & 0.569 & 0.652 & -0.084 & 0.569 & 0.652  \\
 & 2 & 2000 & 0.555 & 0.638 & -0.083 & 0.564 & 0.640  \\
 & 3 & 2000 & 0.560 & 0.638 & -0.078 & 0.576 & 0.652  \\
 & 5 & 2000 & 0.558 & 0.630 & -0.072 & 0.592 & 0.661  \\
 & 8 & 2000 & 0.527 & 0.594 & -0.067 & 0.579 & 0.650  \\
 & 13 & 1230 & 0.544 & 0.567 & -0.023 & 0.614 & 0.673  \\
 & 21 & 761 & 0.514 & 0.496 & \textbf{+0.018} & 0.612 & 0.663  \\
 & 34 & 470 & 0.478 & 0.396 & \textbf{+0.081} & 0.614 & 0.657  \\
 & 50 & 400 & 0.442 & 0.343 & \textbf{+0.099} & 0.618 & 0.672  \\
\midrule
OAS antibody, $\leq$256 aa & 1 & 2000 & 0.900 & 0.942 & -0.041 & 0.900 & 0.942 \\
 & 2 & 2000 & 0.885 & 0.932 & -0.048 & 0.888 & 0.936  \\
 & 3 & 2000 & 0.884 & 0.934 & -0.050 & 0.896 & 0.938  \\
 & 5 & 2000 & 0.881 & 0.935 & -0.053 & 0.902 & 0.942 \\
 & 8 & 2000 & 0.862 & 0.926 & -0.064 & 0.899 & 0.941  \\
 & 13 & 1230 & 0.846 & 0.915 & -0.069 & 0.903 & 0.943  \\
 & 21 & 761 & 0.816 & 0.892 & -0.076 & 0.901 & 0.941  \\
 & 34 & 470 & 0.778 & 0.837 & -0.059 & 0.902 & 0.942 \\
 & 50 & 400 & 0.734 & 0.735 & -0.001 & 0.901 & 0.945  \\
\midrule
native CDRH3 (held-out) & native & 55 & 0.121 & 0.314 & -0.193 & 0.343 & 0.416 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/backbone_validation_sweep.tex <==
% GENERATED by paper/scripts/make_backbone_validation_tables.py -- DO NOT EDIT.
\begin{table}[!htb]
\centering
\caption{Sensitivity of the in-filling DMS score to the length of the scored span, on the 162 assays at most 512 residues. A length-1 span is not the clean analogue of a masked marginal it appears to be: the rearrangement marks the gap with a \emph{single} \texttt{<mask>} whatever the span length, and there is no length token, so at $k=1$ the model is asked for the first residue of an insertion of unknown length rather than for the residue that belongs at that position. Larger $k$ anchors the scored position at the end of the span, so the model has committed to a span of at least $k$; the available context is identical either way. \textbf{The sweep is reported because it measures that concern rather than asserting it away}: the effect is real but small, worth 0.004 of the 0.119 deficit, and it does not account for the gap.}
\label{tab:backbone-validation-sweep}
\small
\begin{tabular}{@{}lrrr@{}}
\toprule
scored span $k$ & in-filling $\rho$ & $\Delta$ vs masked & assays won \\
\midrule
1 \emph{(original)} & +0.2874 & -0.1186 & 23 \\
5 & +0.2887 & -0.1173 & 21 \\
11 & +0.2903 & -0.1157 & 19 \\
25 & +0.2916 & -0.1144 & 20 \\
\midrule
masked baseline & +0.4060 & --- & --- \\
\bottomrule
\end{tabular}
\end{table}


==> tables/logcosh_regime.tex <==
% GENERATED by paper/scripts/make_logcosh_regime_table.py -- DO NOT EDIT.
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Arm & $\beta_\ell(0)$ & $\beta_\ell(T)$ & bowl at $T$ & $\hat{\sigma}$ & residual s.d. \\
\midrule
$M{=}14$, $D{=}4$ & 1.00 & 0.23 & 4.4 & 9.84 & 0.84 \\
$M{=}14$, $D{=}5$ & 1.00 & 0.23 & 4.4 & 9.84 & 0.77 \\
$M{=}9$, $\beta{=}8$ & 1.00 & 0.31 & 3.2 & 9.91 & 1.11 \\
\bottomrule
\end{tabular}


==> tables/logcosh_regime_macros.tex <==
% GENERATED -- DO NOT EDIT. Regenerate: python paper/scripts/make_logcosh_regime_table.py
\newcommand{\lcgamma}{0.999}
\newcommand{\lcsigmazero}{10}
\newcommand{\lccmax}{10}
\newcommand{\lccmin}{2}
\newcommand{\lctau}{875}
\newcommand{\lcbetastart}{1.00}
\newcommand{\lcbetaend}{0.23}
\newcommand{\lcbowlstart}{1.0}
\newcommand{\lcbowlend}{4.4}
\newcommand{\lcsigmahat}{9.84}
\newcommand{\lcsigmahatlo}{9.50}
\newcommand{\lcsigmahathi}{9.99}
\newcommand{\lcsigmapred}{9.82}
\newcommand{\lcdeltastd}{0.84}
\newcommand{\lcvisits}{19}
\newcommand{\lcstepsneeded}{724{,}463}
\newcommand{\lcfoldneeded}{241}
\newcommand{\lcquaderr}{1.9}
\newcommand{\lcquaderrmin}{0.5}
\newcommand{\lcdfourdeltastd}{0.84}
\newcommand{\lcdfoursigmahat}{9.84}
\newcommand{\lcdfourdrift}{1.6}
\newcommand{\lcdfourvisits}{19}
\newcommand{\lcdfournpdbs}{618}
\newcommand{\lcdfourntasks}{4}
\newcommand{\lcdfourtrainsteps}{3{,}000}
\newcommand{\lcdfourtaufrac}{29}
\newcommand{\lcdfourbetastart}{1.00}
\newcommand{\lcdfourbetaend}{0.23}
\newcommand{\lcdfourbowlstart}{1.0}
\newcommand{\lcdfourbowlend}{4.4}
\newcommand{\lcdfourkneestart}{1.19}
\newcommand{\lcdfourkneeend}{5.18}
\newcommand{\lcdfourtailstart}{23}
\newcommand{\lcdfourtailend}{0.0}
\newcommand{\lcdfivedeltastd}{0.77}
\newcommand{\lcdfivesigmahat}{9.84}
\newcommand{\lcdfivedrift}{1.6}
\newcommand{\lcdfivevisits}{20}
\newcommand{\lcdfivenpdbs}{610}
\newcommand{\lcdfiventasks}{4}
\newcommand{\lcdfivetrainsteps}{3{,}000}
\newcommand{\lcdfivetaufrac}{29}
\newcommand{\lcdfivebetastart}{1.00}
\newcommand{\lcdfivebetaend}{0.23}
\newcommand{\lcdfivebowlstart}{1.0}
\newcommand{\lcdfivebowlend}{4.4}
\newcommand{\lcdfivekneestart}{1.31}
\newcommand{\lcdfivekneeend}{5.68}
\newcommand{\lcdfivetailstart}{19}
\newcommand{\lcdfivetailend}{0.0}
\newcommand{\lcbeightdeltastd}{1.11}
\newcommand{\lcbeightsigmahat}{9.91}
\newcommand{\lcbeightdrift}{0.9}
\newcommand{\lcbeightvisits}{11}
\newcommand{\lcbeightnpdbs}{613}
\newcommand{\lcbeightntasks}{4}
\newcommand{\lcbeighttrainsteps}{1{,}750}
\newcommand{\lcbeighttaufrac}{50}
\newcommand{\lcbeightbetastart}{1.00}
\newcommand{\lcbeightbetaend}{0.31}
\newcommand{\lcbeightbowlstart}{1.0}
\newcommand{\lcbeightbowlend}{3.2}
\newcommand{\lcbeightkneestart}{0.90}
\newcommand{\lcbeightkneeend}{2.91}
\newcommand{\lcbeighttailstart}{37}
\newcommand{\lcbeighttailend}{0.4}
\newcommand{\lcvisitslo}{11}
\newcommand{\lcvisitshi}{20}
\newcommand{\lcarmsigmahatlo}{9.84}
\newcommand{\lcarmsigmahathi}{9.91}
\newcommand{\lcarmdeltalo}{0.77}
\newcommand{\lcarmdeltahi}{1.11}
\newcommand{\lcallsigmalo}{9.50}
\newcommand{\lcallsigmahi}{9.99}
\newcommand{\lcdriftmax}{1.6}
\newcommand{\lcstepsneededmin}{671{,}996}
\newcommand{\lcfoldneededmin}{241}
\newcommand{\lcfoldneededmax}{384}
\newcommand{\lcswonedeltastd}{0.13}
\newcommand{\lcswonekneestart}{7.86}
\newcommand{\lcswonekneeend}{25.50}
\newcommand{\lcswonetailstart}{0}
\newcommand{\lcswonesaturated}{0}
\newcommand{\lcsweightdeltastd}{0.86}
\newcommand{\lcsweightkneestart}{1.17}
\newcommand{\lcsweightkneeend}{3.78}
\newcommand{\lcsweighttailstart}{24}
\newcommand{\lcsweightsaturated}{3}
\newcommand{\lcswthirtytwodeltastd}{4.72}
\newcommand{\lcswthirtytwokneestart}{0.21}
\newcommand{\lcswthirtytwokneeend}{0.69}
\newcommand{\lcswthirtytwotailstart}{83}
\newcommand{\lcswthirtytwosaturated}{68}
\newcommand{\lcswgradone}{0.81}
\newcommand{\lcswgradtwo}{0.55}
\newcommand{\lcswgradthree}{0.38}
\newcommand{\lcswtrainsteps}{1{,}750}
\newcommand{\lcswspreadratio}{37}
\newcommand{\lcdfourfoldtothirtytwo}{5.6}


==> tables/lr_sweep_fullscale.tex <==
% GENERATED by paper/scripts/make_sweep_tables.py -- DO NOT EDIT.
% Regenerate:  python paper/scripts/make_sweep_tables.py beta --check
% git 8959be3; runs 5e-5=mcawr8cr, 1e-4=9kjf0gxh, 2e-4=f17awz35, 3e-4=yds65tku, 5e-4=upjtl3d3, 1e-3=3tjhom0y, 2e-3=tak82cl4
\begin{tabular}{@{}lccccccc@{}}
\toprule
statistic & $\eta = 5e-5$ & $\eta = 1e-4$ & $\eta = 2e-4$ & $\eta = 3e-4$ & $\eta = 5e-4$ & $\eta = 1e-3$ & $\eta = 2e-3$ \\
\midrule
trajectory-balance residual spread (final) & 0.151 & 0.127 & 0.109 & 0.128 & 0.173 & 0.199 & 0.263 \\
\quad relative change, last 40\% of training & -6.4\% & -4.5\% & -5.8\% & -8.7\% & -1.7\% & -4.3\% & +2.9\% \\
hypervolume (final) & 0.329 & 0.503 & 0.615 & 0.499 & 0.377 & 0.506 & 0.353 \\
hypervolume (best) & 0.649 & 0.831 & 0.678 & 0.542 & 0.531 & 0.583 & 0.634 \\
mean sampled reward (final) & 0.628 & 0.629 & 0.630 & 0.623 & 0.620 & 0.626 & 0.618 \\
optimizer steps logged & 2434 & 2028 & 1906 & 2387 & 2232 & 2480 & 2140 \\
run state & finished & finished & finished & finished & finished & finished & crashed \\
\bottomrule
\end{tabular}


==> tables/postfilter_diversity_cascade.tex <==
% GENERATED by paper/scripts/postfilter_analysis.py tables -- DO NOT EDIT.
% Regenerate:  python paper/scripts/postfilter_analysis.py tables

% Diversity at CDRH3 identity 0.4, deliberately BELOW the 0.50 the B3
% budget deduplicates at: at >= 0.50 every arm is pinned at 1.000 clusters per
% design from B3 onward, and the statistic cannot express a difference at all.
% Clus./design is comparable ACROSS ARMS within a stage, never across stages
% (cluster counts grow sublinearly in n). Retention is comparable across both:
% clusters are defined once on the pool and every stage scored against that partition.
\begin{tabular}{@{}llcccccc@{}}
\toprule
Arm & Stage & $n$ & Unique & Entropy (bits) & Clus./design & Pool clus.\ retained & Vendi \\
\midrule
GFN D=4 & Pool & 32,768 & 1.000 & 4.23 & 0.340 & 1.000 & 1.22 \\
GFN D=4 & Stage 0 & 23,556 & 1.000 & 4.17 & 0.356 & 0.872 & 1.22 \\
GFN D=4 & B3 (1k) & 1,000 & 1.000 & 3.99 & 0.741 & 0.077 & 1.22 \\
GFN D=4 & B4 (250) & 250 & 1.000 & 3.86 & 0.880 & 0.021 & 1.20 \\
GFN D=5 & Pool & 32,768 & 1.000 & 4.24 & 0.356 & 1.000 & 1.22 \\
GFN D=5 & Stage 0 & 22,722 & 1.000 & 4.18 & 0.377 & 0.852 & 1.22 \\
GFN D=5 & B3 (1k) & 1,000 & 1.000 & 4.00 & 0.774 & 0.077 & 1.21 \\
GFN D=5 & B4 (250) & 250 & 1.000 & 3.89 & 0.900 & 0.020 & 1.20 \\
GFN Fixed & Pool & 32,768 & 1.000 & 4.21 & 0.339 & 1.000 & 1.22 \\
GFN Fixed & Stage 0 & 15,840 & 1.000 & 4.14 & 0.400 & 0.733 & 1.21 \\
GFN Fixed & B3 (1k) & 1,000 & 1.000 & 3.98 & 0.730 & 0.079 & 1.21 \\
GFN Fixed & B4 (250) & 250 & 1.000 & 3.86 & 0.876 & 0.021 & 1.20 \\
Random Baseline & Pool & 32,768 & 1.000 & 4.32 & 0.431 & 1.000 & 1.22 \\
Random Baseline & Stage 0 & 15,768 & 1.000 & 4.25 & 0.515 & 0.691 & 1.22 \\
Random Baseline & B3 (1k) & 1,000 & 1.000 & 4.10 & 0.854 & 0.065 & 1.21 \\
Random Baseline & B4 (250) & 250 & 1.000 & 4.01 & 0.940 & 0.017 & 1.21 \\
AMPLIFY Prior & Pool & 32,716 & 1.000 & 3.45 & 0.049 & 1.000 & 1.22 \\
AMPLIFY Prior & Stage 0 & 26,559 & 1.000 & 3.43 & 0.052 & 0.911 & 1.22 \\
AMPLIFY Prior & B3 (1k) & 1,000 & 1.000 & 3.51 & 0.333 & 0.336 & 1.22 \\
AMPLIFY Prior & B4 (250) & 250 & 1.000 & 3.41 & 0.496 & 0.117 & 1.21 \\
ProteinMPNN & Pool & 32,750 & 1.000 & 2.67 & 0.016 & 1.000 & 1.16 \\
ProteinMPNN & Stage 0 & 23,989 & 1.000 & 2.67 & 0.023 & 0.906 & 1.16 \\
ProteinMPNN & B3 (1k) & 1,000 & 1.000 & 3.23 & 0.281 & 0.581 & 1.18 \\
ProteinMPNN & B4 (250) & 250 & 1.000 & 3.12 & 0.420 & 0.244 & 1.17 \\
ESM-IF & Pool & 32,660 & 1.000 & 2.75 & 0.026 & 1.000 & 1.17 \\
ESM-IF & Stage 0 & 23,859 & 1.000 & 2.75 & 0.028 & 0.913 & 1.17 \\
ESM-IF & B3 (1k) & 1,000 & 1.000 & 3.29 & 0.295 & 0.482 & 1.19 \\
ESM-IF & B4 (250) & 250 & 1.000 & 3.13 & 0.432 & 0.189 & 1.19 \\
\bottomrule
\end{tabular}


==> tables/postfilter_pareto_fronts.tex <==
% GENERATED by paper/scripts/postfilter_analysis.py tables -- DO NOT EDIT.
% Regenerate:  python paper/scripts/postfilter_analysis.py tables

% Body of tab:pareto-pooled. Space=4d, stage=pool, per-target MEDIANS
% over 45 targets; median joint front = 437 points/target.
% Computed on the COMMON RAW SCALE -- an earlier version mixed normalizer states
% across arms, which forces the inverse-folding arms to zero on units alone.
\begin{tabular}{@{}lcc@{}}
\toprule
Arm & own front & share of the JOINT front \\
\midrule
GFN D=4 & 135 & 17 \\
GFN D=5 & 142 & 11 \\
GFN Fixed & 138 & 28 \\
Random Baseline & 124 & 2 \\
AMPLIFY Prior & 212 & 202 \\
ProteinMPNN & 148 & 38 \\
ESM-IF & 161 & 101 \\
\bottomrule
\end{tabular}


==> tables/postfilter_summary_diff.tex <==
% GENERATED by paper/scripts/make_postfilter_summary_table.py -- DO NOT EDIT.
% Regenerate: ./experiments/sbatch_cluster.sh experiments/make_postfilter_summary_table.sh
% Supersedes stage2_sap.tex, stage4_binding.tex, agreement_confidence.tex --
% one row per arm, over the merged 45-target x 7-arm corpus.
% SAP median is POOLED across a arm's designs; SAP depth and every other family
% are computed WITHIN each target then averaged, so no single target dominates.
% Stage 3 RMSD is the ABB3<->Chai agreement RMSD and pLDDT is the Chai CDR-H3
% pLDDT, both median-within-target; rho is their rank correlation and Retained
% the share of the pLDDT top 250 inside the best-25% RMSD (independence: 25%).
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lr rrr rrrr rrrrr@{}}
\toprule
& Stage 0 (45) & \multicolumn{3}{c}{Stage 2 --- CDR-H3 SAP (45)} & \multicolumn{4}{c}{Stage 3 --- fold agreement (45)} & \multicolumn{5}{c}{Stage 4 --- binding $\Delta\Delta G$ (45)} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-5}\cmidrule(lr){6-9}\cmidrule(lr){10-14}
Arm & Surv.\ & Median & Best 10\% & Won & RMSD (\AA) & pLDDT & $\rho$ & Retained & FoldX & Rosetta & FoldX IMP & Rosetta IMP & $\rho$ \\
\midrule
\textcolor{red}{GFN} $D{=}4$ & 71.1\% & $-0.0088$ & $-0.0877$ & 0/45 & $3.54$ & $77.7$ & $-0.351$ & 40.6\% & $-4.96$ & $-8.88$ & 23.1\% & 17.2\% & $+0.47$ \\
\textcolor{red}{GFN} $D{=}5$ & 68.3\% & $-0.0116$ & $-0.0886$ & 0/45 & $3.65$ & $77.1$ & $-0.340$ & 40.2\% & $-5.50$ & $-9.73$ & 24.0\% & 17.5\% & $+0.46$ \\
\textcolor{red}{GFN Fixed} & 47.1\% & $-0.0200$ & $-0.0959$ & 40/45 & $3.55$ & $77.6$ & $-0.359$ & 40.1\% & $-4.78$ & $-9.31$ & 22.7\% & 16.8\% & $+0.46$ \\
\midrule
Random baseline & 46.0\% & $+0.0177$ & $-0.0619$ & 0/45 & $3.87$ & $76.0$ & $-0.283$ & 39.6\% & $-5.48$ & $-9.34$ & 24.0\% & 18.0\% & $+0.47$ \\
AMPLIFY prior & 80.1\% & $+0.0271$ & $-0.0443$ & 0/45 & $2.94$ & $80.4$ & $-0.337$ & 36.5\% & $-5.09$ & $-9.34$ & 24.2\% & 19.6\% & $+0.47$ \\
ProteinMPNN & 68.7\% & $+0.0138$ & $-0.0514$ & 2/45 & $3.02$ & $82.0$ & $-0.331$ & 35.0\% & $-6.20$ & $-14.52$ & 30.4\% & 24.6\% & $+0.52$ \\
ESM-IF & 72.1\% & $+0.0096$ & $-0.0587$ & 3/45 & $3.18$ & $80.6$ & $-0.297$ & 35.9\% & $-6.09$ & $-13.07$ & 27.7\% & 23.3\% & $+0.50$ \\
\bottomrule
\end{tabular}%
}


==> tables/postfilter_tails.tex <==
% GENERATED by paper/scripts/postfilter_analysis.py tables -- DO NOT EDIT.
% Regenerate:  python paper/scripts/postfilter_analysis.py tables

% Tail behaviour at B3 (1k), median over targets.
% Top-1\% lift: share of the six-arm pooled best 1\% within a target, divided by
% the share the arm's raw count alone would earn. 1.00 = exactly proportional.
\begin{tabular}{@{}llcccc@{}}
\toprule
Metric & Arm & Median & Fav.\ 5\% quantile & $E[\text{best of }100]$ & Top-1\% lift \\
\midrule
hard liabilities & GFN D=4 & 0.00 & 0.00 & 0.00 & 1.00 \\
hard liabilities & GFN D=5 & 0.00 & 0.00 & 0.00 & 1.00 \\
hard liabilities & GFN Fixed & 0.00 & 0.00 & 0.00 & 1.00 \\
hard liabilities & Random Baseline & 0.00 & 0.00 & 0.00 & 1.00 \\
hard liabilities & AMPLIFY Prior & 0.00 & 0.00 & 0.00 & 1.00 \\
hard liabilities & ProteinMPNN & 0.00 & 0.00 & 0.00 & 1.00 \\
hard liabilities & ESM-IF & 0.00 & 0.00 & 0.00 & 1.00 \\
soft liabilities & GFN D=4 & 1.00 & 0.00 & 0.00 & 1.16 \\
soft liabilities & GFN D=5 & 1.00 & 0.00 & 0.00 & 1.12 \\
soft liabilities & GFN Fixed & 1.00 & 0.00 & 0.00 & 0.83 \\
soft liabilities & Random Baseline & 1.00 & 0.00 & 0.00 & 0.57 \\
soft liabilities & AMPLIFY Prior & 1.00 & 0.00 & 0.00 & 1.34 \\
soft liabilities & ProteinMPNN & 1.00 & 0.00 & 0.00 & 1.03 \\
soft liabilities & ESM-IF & 1.00 & 0.00 & 0.00 & 0.99 \\
scRMSD & GFN D=4 & 2.49 & 1.80 & 1.49 & 0.50 \\
scRMSD & GFN D=5 & 2.50 & 1.78 & 1.41 & 0.50 \\
scRMSD & GFN Fixed & 2.48 & 1.80 & 1.46 & 0.50 \\
scRMSD & Random Baseline & 2.44 & 1.82 & 1.46 & 0.40 \\
scRMSD & AMPLIFY Prior & 2.43 & 1.65 & 1.32 & 0.70 \\
scRMSD & ProteinMPNN & 2.35 & 1.47 & 1.20 & 2.10 \\
scRMSD & ESM-IF & 2.34 & 1.45 & 1.11 & 1.60 \\
ABB3 pLDDT & GFN D=4 & 87.94 & 89.37 & 90.27 & 1.00 \\
ABB3 pLDDT & GFN D=5 & 87.83 & 89.37 & 90.21 & 0.80 \\
ABB3 pLDDT & GFN Fixed & 87.30 & 89.12 & 89.98 & 0.60 \\
ABB3 pLDDT & Random Baseline & 87.42 & 89.07 & 90.02 & 0.30 \\
ABB3 pLDDT & AMPLIFY Prior & 86.70 & 89.41 & 90.54 & 2.03 \\
ABB3 pLDDT & ProteinMPNN & 85.34 & 88.64 & 89.56 & 0.60 \\
ABB3 pLDDT & ESM-IF & 84.93 & 88.57 & 89.84 & 0.90 \\
Chai pLDDT & GFN D=4 & 78.76 & 88.42 & 91.90 & 0.70 \\
Chai pLDDT & GFN D=5 & 78.52 & 88.40 & 92.21 & 0.60 \\
Chai pLDDT & GFN Fixed & 79.12 & 88.86 & 91.98 & 0.60 \\
Chai pLDDT & Random Baseline & 77.16 & 87.37 & 91.61 & 0.30 \\
Chai pLDDT & AMPLIFY Prior & 80.67 & 89.55 & 92.70 & 1.20 \\
Chai pLDDT & ProteinMPNN & 82.76 & 91.14 & 93.38 & 2.10 \\
Chai pLDDT & ESM-IF & 81.88 & 90.02 & 92.91 & 1.30 \\
agreement RMSD & GFN D=4 & 3.32 & 1.54 & 1.14 & 0.90 \\
agreement RMSD & GFN D=5 & 3.38 & 1.61 & 1.09 & 0.80 \\
agreement RMSD & GFN Fixed & 3.23 & 1.57 & 1.09 & 0.80 \\
agreement RMSD & Random Baseline & 3.72 & 1.70 & 1.25 & 0.50 \\
agreement RMSD & AMPLIFY Prior & 2.62 & 1.36 & 1.02 & 1.70 \\
agreement RMSD & ProteinMPNN & 2.64 & 1.39 & 0.97 & 1.20 \\
agreement RMSD & ESM-IF & 2.73 & 1.39 & 1.04 & 0.90 \\
agreement lDDT & GFN D=4 & 0.74 & 0.86 & 0.90 & 1.00 \\
agreement lDDT & GFN D=5 & 0.73 & 0.85 & 0.90 & 0.80 \\
agreement lDDT & GFN Fixed & 0.73 & 0.85 & 0.90 & 0.80 \\
agreement lDDT & Random Baseline & 0.72 & 0.84 & 0.88 & 0.50 \\
agreement lDDT & AMPLIFY Prior & 0.77 & 0.87 & 0.91 & 1.60 \\
agreement lDDT & ProteinMPNN & 0.78 & 0.87 & 0.91 & 1.10 \\
agreement lDDT & ESM-IF & 0.77 & 0.87 & 0.90 & 0.90 \\
\bottomrule
\end{tabular}


==> tables/run_comparison_axes.tex <==
% GENERATED by paper/scripts/make_run_comparison_tables.py -- DO NOT EDIT.
\begin{table}[!htb]
\centering
\caption{Per-axis selectivity, within each arm, on the vertex-inclusive sweeps. \texttt{on-target} is the response averaged over objectives weighted by the axis, \texttt{off-target} over the complement, and selectivity their difference; \texttt{alignment} is the Spearman correlation between what the axis weights and what actually moves. \textbf{The axis$\to$objective weighting is the trained matrix $A$ for \textsc{expanded14}, read from the checkpoint} --- it is not recoverable from the saved preferences, because under a learned projection the eval writes the reference directions as an independent draw (measured relative residual 0.74 against 0.00 for group expansion), and regressing on it returns a near-uniform matrix that forces every selectivity to $\approx$0. Each arm's null is its own base policy. Rows are within-arm diagnostics and are \emph{not} comparable across arms; the cross-arm number is Table~\ref{tab:run-comparison-controllability}.}
\label{tab:run-comparison-axes}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llrrrl@{}}
\toprule
& axis & on-target & off-target & selectivity & top-responding objective \\
\midrule
\textsc{expanded14} & slot0 & 0.347 & 0.025 & 0.322 & \texttt{stability\_esm\_if} \\
 & slot1 & 0.367 & -0.404 & 0.771 & \texttt{mhc2} \\
 & slot2 & 0.483 & -0.135 & 0.619 & \texttt{developability} \\
 & slot3 & 0.422 & 0.000 & 0.422 & \texttt{naturalness} \\
 & slot4 & 0.471 & 0.158 & 0.313 & \texttt{sequence\_liability} \\
 & \emph{null (base policy)} & & & \emph{-0.033 to +0.039} & \\
\midrule
\textsc{scaffold} & mhc2 & 0.598 & -0.810 & 1.408 & \texttt{mhc2} \\
 & developability & 0.879 & 0.269 & 0.610 & \texttt{developability} \\
 & naturalness & 0.484 & 0.182 & 0.302 & \texttt{naturalness} \\
 & stability & 0.204 & -0.233 & 0.436 & \texttt{stability\_boltzif} \\
 & \emph{null (base policy)} & & & \emph{-0.053 to +0.281} & \\
\bottomrule
\end{tabular}
\end{table}


==> tables/run_comparison_controllability.tex <==
% GENERATED by paper/scripts/make_run_comparison_tables.py -- DO NOT EDIT.
\begin{table}[!htb]
\centering
\caption{Steerability, measured without reference to the preference axes. Each arm is swept over a \textbf{vertex-inclusive simplex grid} in its own conditioning space (126 points at $D{=}5$, 120 at $D{=}4$ --- the closest matched pair the lattice allows, both containing every vertex) and scored against \textbf{its own base-policy null}, the same backbone handed the same preferences but unable to act on them. The null is not a formality: it is the noise floor at this $(n_\mathrm{prefs}, n_\mathrm{samples}, D)$, it differs per arm, and a per-preference mean over finite samples produces nonzero span and energy on its own. Per-axis selectivity is deliberately \emph{not} used for the cross-arm comparison: \texttt{off\_target} averages over 9 versus 14 objectives, the simplex confound scales with $D$, and one arm's axes are config groups while the other's are learned slots. \textbf{Effective rank inverts}: the null scores 7.1--7.3 of 9 because isotropic noise fills every dimension, so a structured response scores \emph{lower}; between trained arms the raw value carries the comparison.}
\label{tab:run-comparison-controllability}
\small
\begin{tabular}{@{}llrrrr@{}}
\toprule
& & trained & null & ratio & $p$ vs null \\
\midrule
\textsc{expanded14} & reachable span & 0.1260 & 0.0786 & 1.603 & 0.0156$^{*}$ \\
 & steering energy & 0.0967 & 0.0469 & 2.059 & 0.0078$^{**}$ \\
 & effective rank & 4.3920 & 7.3001 & 0.602 & 0.0078$^{**}$ \\
\midrule
\textsc{scaffold} & reachable span & 0.1338 & 0.0858 & 1.560 & 0.0391$^{*}$ \\
 & steering energy & 0.1120 & 0.0547 & 2.048 & 0.0078$^{**}$ \\
 & effective rank & 4.0003 & 7.0866 & 0.564 & 0.0078$^{**}$ \\
\midrule
\multicolumn{6}{@{}l}{\emph{head-to-head, noise-normalised, paired over 8 targets}} \\
\quad reachable span & & 1.609 & 1.562 & +0.047 & $p=0.55$ \\
\quad steering energy & & 2.059 & 2.125 & -0.067 & $p=0.95$ \\
\quad effective rank & & 0.604 & 0.569 & +0.034 & $p=0.11$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/run_comparison_pool.tex <==
% GENERATED by paper/scripts/make_run_comparison_tables.py -- DO NOT EDIT.
\begin{table}[!htb]
\centering
\caption{Pool quality on the 45 held-out RAbD test targets, paired. Both arms generate 32{,}768 designs per target and are scored by the same oracles; metrics are recomputed here over the \textbf{intersection} of the arms' objective sets (the 9 that \textsc{scaffold} trains on, a strict subset of \textsc{expanded14}'s 14), so neither is credited for an objective the other never saw. \textbf{The training-time numbers cannot be differenced instead}: hypervolume is measured in each run's own reward space, 9-d and 14-d hypervolumes are different units, and an easy extra objective raises the figure on its own. The base policy column is the same backbone with no GFlowNet training, handed identical preferences. $p$ from a paired Wilcoxon signed-rank test over targets ($^{*}p<0.05$, $^{**}p<0.01$, $^{***}p<0.001$). Pareto count is a \emph{shape} statistic, not a quality one --- a pool concentrated in a high-reward region has fewer non-dominated points than a diffuse one.}
\label{tab:run-comparison-pool}
\small
\begin{tabular}{@{}lrrrrr@{}}
\toprule
& \textsc{expanded14} & \textsc{scaffold} & base policy & $\Delta$ & wins \\
\midrule
hypervolume (4 groups) & 0.8746 & 0.8651 & 0.6031 & +0.0095$^{**}$ & 32/45 \\
mean reward, 9 shared objectives & 0.5097 & 0.5064 & 0.4193 & +0.0033$^{**}$ & 31/45 \\
diversity (mean pairwise edit distance) & 12.050 & 12.021 & 12.147 & +0.029$^{***}$ & 41/45 \\
unique designs & 32604 & 32554 & 32518 & +50 & 3/45 \\
Pareto points (4 groups) & 89.2 & 103.4 & 125.2 & -14.3$^{*}$ & 17/45 \\
\midrule
\multicolumn{6}{@{}l}{\emph{per-objective mean reward}} \\
\quad mhc2 & 0.6393 & 0.6683 & 0.6125 & -0.0290$^{***}$ & 0/45 \\
\quad developability & 0.3218 & 0.3149 & 0.1390 & +0.0068 & 25/45 \\
\quad naturalness & 0.5049 & 0.5007 & 0.4167 & +0.0042$^{**}$ & 29/45 \\
\quad stability\_esm\_if & 0.6252 & 0.5975 & 0.5079 & +0.0278$^{***}$ & 45/45 \\
\quad stability\_proteinmpnn\_vanilla & 0.4690 & 0.4660 & 0.3980 & +0.0030$^{*}$ & 29/45 \\
\quad stability\_proteinmpnn\_soluble & 0.4608 & 0.4629 & 0.3949 & -0.0022 & 22/45 \\
\quad stability\_proteinmpnn\_antibody & 0.4578 & 0.4820 & 0.3769 & -0.0243$^{***}$ & 0/45 \\
\quad stability\_proteinmpnn\_ca\_only & 0.4910 & 0.4471 & 0.4156 & +0.0439$^{***}$ & 45/45 \\
\quad stability\_boltzif & 0.6180 & 0.6186 & 0.5124 & -0.0005 & 23/45 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/run_comparison_projection.tex <==
% GENERATED by paper/scripts/make_run_comparison_tables.py -- DO NOT EDIT.
\begin{table}[!htb]
\centering
\caption{The learned reward projection $A$ of \textsc{expanded14}, $\mathrm{softmax}(\text{logits})$ over 14 objectives, aggregated to the 9 config groups (rows sum to 1). Read from the checkpoint's \texttt{target} copy, which is what generates rewards; the optimised \texttt{learner} copy lags it by an EMA time constant (measured max difference 0.022). \textbf{Nothing supplied the grouping}: the five slots separate the six stability oracles, MHC-II, and developability-with-novelty on their own, and slot~3 pools the three sequence-likelihood oracles (\texttt{naturalness}, \texttt{h3berta}, \texttt{ablang2}) in near-equal thirds --- which is evidence they are interchangeable \emph{as a steering direction}, whatever they measure individually. Every slot's entropy is well below uniform (2.64 nats).}
\label{tab:run-comparison-projection}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrrrrr@{}}
\toprule
slot & \rotatebox{60}{\texttt{mhc2}} & \rotatebox{60}{\texttt{devel.}} & \rotatebox{60}{\texttt{naturalness}} & \rotatebox{60}{\texttt{stability}} & \rotatebox{60}{\texttt{liability}} & \rotatebox{60}{\texttt{train-nov.}} & \rotatebox{60}{\texttt{blosum-nov.}} & \rotatebox{60}{\texttt{h3berta}} & \rotatebox{60}{\texttt{ablang2}} & entropy \\
\midrule
0 & 0.00 & 0.16 & 0.00 & \textbf{0.83} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 2.00 \\
1 & \textbf{0.73} & 0.07 & 0.02 & 0.08 & 0.01 & 0.01 & 0.00 & 0.04 & 0.04 & 1.19 \\
2 & 0.01 & \textbf{0.52} & 0.01 & 0.04 & 0.03 & 0.18 & 0.19 & 0.01 & 0.01 & 1.46 \\
3 & 0.00 & 0.05 & 0.24 & 0.19 & 0.00 & 0.00 & 0.00 & 0.25 & 0.25 & 1.73 \\
4 & 0.01 & \textbf{0.31} & 0.06 & 0.15 & \textbf{0.42} & 0.00 & 0.00 & 0.02 & 0.03 & 1.70 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/selection_ranker.tex <==
% GENERATED by paper/scripts/make_selection_ranker_tables.py -- DO NOT EDIT.
% Regenerate: ./experiments/sbatch_cluster.sh experiments/make_selection_ranker_tables.sh
%   then copy $SCRATCH/outputs/selection_ranker/* into paper/tables/ from a LOGIN node.
% PAIRED WITHIN (arm, target); pooling ddG across targets would repeat the
% tab:pareto-pooled defect (different energy scales per interface).
% Contrast is between the DISJOINT selections; shared designs carry no signal.
% Positive Delta and positive Cliff's delta both mean B4 binds tighter.
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
& & & \multicolumn{2}{c}{Rosetta} & \multicolumn{2}{c}{FoldX} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Arm & Units & Jaccard & $\Delta$ (REU) & $\delta$ & $\Delta$ (kcal/mol) & $\delta$ \\
\midrule
AbGFN $D{=}4$ & 20 & 0.259 & $+1.247$ & $+0.100$ & $+0.245$ & $+0.032$ \\
AbGFN $D{=}5$ & 20 & 0.256 & $+1.477$ & $+0.146$ & $+0.244$ & $+0.046$ \\
AbGFN $\beta{=}8$ & 28 & 0.265 & $+0.883$ & $+0.107$ & $+0.345$ & $+0.068$ \\
Uniform random & 28 & 0.266 & $+1.501$ & $+0.132$ & $+0.290$ & $+0.044$ \\
ProteinMPNN & 20 & 0.221 & $-0.112$ & $-0.002$ & $-0.205$ & $-0.034$ \\
ESM-IF & 20 & 0.234 & $+0.912$ & $+0.086$ & $+0.065$ & $+0.032$ \\
\midrule
All & 136 & 0.252 & $+1.143$ & $+0.106$ & $+0.245$ & $+0.044$ \\
\bottomrule
\end{tabular}


==> tables/selection_ranker_macros.tex <==
% GENERATED by paper/scripts/make_selection_ranker_tables.py -- DO NOT EDIT.
\newcommand{\srUnits}{136}
\newcommand{\srDesigns}{54{,}475}
\newcommand{\srJaccard}{0.252}
\newcommand{\srDeltaRosetta}{+1.143}
\newcommand{\srDeltaFoldx}{+0.245}
\newcommand{\srCliffRosetta}{+0.106}
\newcommand{\srCliffFoldx}{+0.044}
\newcommand{\srWinRosetta}{91/136}
\newcommand{\srWinFoldx}{83/136}
\newcommand{\srPRosetta}{4.6\times10^{-5}}
\newcommand{\srPFoldx}{0.0019}

